Adaptive Diffusion Models for Sparse-View Motion-Corrected Head Cone-beam CT

Cone-beam computed tomography (CBCT) is an imaging modality widely used in head and neck diagnostics due to its accessibility and lower radiation dose. However, its relatively long acquisition times make it susceptible to patient motion, especially under sparse-view settings used to reduce dose, which can result in severe image artifacts. In this work, we propose a novel framework combining joint reconstruction and motion estimation (JRM) with an adaptive diffusion model (ADM) that simultaneously addresses motion compensation and sparse-view reconstruction in head CBCT. Leveraging recent advances in diffusion-based generative models, our method integrates a wavelet-domain diffusion prior into an iterative reconstruction pipeline to guide the solution toward anatomically plausible volumes while estimating rigid motion parameters in a blind fashion. We evaluate our method on simulated motion-affected CBCT data derived from real clinical computed tomography (CT) volumes. Experimental results demonstrate that JRM- ADM achieves consistent quantitative improvements over both traditional and learning-based baselines. In highly undersampled cases, JRM-ADM improves peak signal-to-noise ratio (PSNR) by more than 4 dB and structural similarity index measure (SSIM) by 0.10 compared to the baseline motion-corrected (MC) reconstruction method. These results highlight the potential of our approach to enable motion-robust, low-dose CBCT imaging, paving the way for improved clinical viability. The project page is available at https://antoinedepaepe.github.io/jrm-adm-io/.

==> content/old.tex <==
%$\boldcalA_{\boldc} \triangleq \left[{\boldcalA_{\boldc}^1}\transp, \cdots, {\boldcalA_{\boldc}^{n_\rmt}}\transp\right]\transp  \colon \calX \to \calY^{n_\rmt}$ where $\boldcalA_{\boldc}^k = \boldcalR_k\circ \boldcalW_{\boldvarphi_k}\colon \calX\to\calY$, the negative log-posterior is approximated as (see \citeauthor{elbakri2002statistical}~\cite{elbakri2002statistical})
%\begin{equation}\label{eq:neglogpost}
%	-\log p(\boldy \mid \boldx, \boldc) \approx \frac{1}{2}  \| \boldcalA_{\boldc}(\boldx) - \boldb \|_{\boldW}^2
%\end{equation}
%where $\boldb = \{\boldb_k\}_{k=1}^{n_{\rmt}} \in \calY^{n_\rmt}$, $\boldb_k = [b_{1,k},\dots,b_{n,k}]\transp$ with $b_{i,k} \triangleq \log I/y_{i,k}$, 
%and $\boldW \in \R^{n\cdot n_{\rma}\times n\cdot n_{\rma}}_+$ is a diagonal matrix of statistical weights. 
%An alternative to \eqref{eq:map} is therefore the standard \ac{JRM} approach
%\begin{equation}\label{eq:jrm}
%	\min_{\boldx \in \calX, \boldc \in \boldcalC }  \,  \frac{1}{2}  \| \boldcalA_{\boldphi}(\boldx) - \boldb \|_{\boldW}^2   +   \gamma R(\boldx)
%\end{equation}  
%where  $R\colon\calX\to \R$ is a convex regularizer that replaces the unknown prior $-\log p (\boldx)$ and $\gamma>0$ is a weight. 




% figures/methods/motion_sv/gt_depth.png
% figures/methods/motion_sv/motion_only_depth.png
% figures/methods/motion_sv/motion_sparse_view_noise_depth.png
% figures/methods/motion_sv/sparse_view_noise_only_depth.png


% Applying \acp{DM} to \ac{3D} medical imaging is challenging due to high computational cost and memory usage. \Acp{LDM} take into account these challenges by operating in a ``compressed''  space. Recent works proposed to perform the diffusion in a the wavelet domain \cite{friedrich2024wdm}, significantly reducing memory usage during training and inference while achieving state-of-the-art performance. In that context, an orthogonal \ac{DWT} $\boldcalV \colon \calX \to \calV \triangleq \R^{8 \times \frac{n_x}{2} \times \frac{n_y}{2} \times \frac{n_z}{2} }$, with $\boldcalV^{-1} = \boldcalV\transp $, is utilized to decompose a \ac{3D} image $\boldx$ into a 8-channel wavelet coefficients \ac{3D} image $\boldw$ with half the spatial dimension of $\boldx$. The orthogonality of the choosen \ac{DWT} allows us to switch from the wavelet domain represenation to image one, and so on. 

% In fact, the diffusion process in \ref{eq:xtfromx0} can be rewriten as $\boldcalV\boldx_{t} = \sqrt{\alpha_t} \boldcalV\boldx_{t-1}  + (1-\alpha_t) \boldcalV \boldepsilon$, with $\boldepsilon \sim \calN(\boldzero_{\calX}, \boldI_{\calX})$, and since the \ac{DWT} is orthogonal, we are assured that $\boldcalV \boldepsilon \sim \calN(\boldzero_{\calX}$ also. Same reasoning can be applied for the reverse process.

% Then, training an \ac{NN} $\hat{\boldw}_{\boldtheta} \colon \calV \times [0,T]\to \calV$ to recover $\boldw_0$ from $\boldw_t$ wavelet domain is equivalent to train an \ac{NN} $\boldx_{\boldtheta}  \colon \calX \times [0,T]\to \calX$ to recover $\boldx_{0}$ from $\boldx_{t}$ in the image domain. 

% Following this, the \ac{NN} is train in the wavelet domain $\calV$, and switching from one domain to another is allow.

%\begin{align*}\label{eq:tweedie_cond}
%	\mathbb{E}\left[ \boldx_{0} \mid\boldx_t, \boldy\right] & = \boldx_{t} + \sigma_{t}^2 \nabla \log p_t(\boldx_t| \boldy)\\
%	& = \boldx_{t} +  \sigma_{t}^2 \nabla_{\boldx_t} \log p_t(\boldx_t) + \sigma_{t}^2 \nabla_{\boldx_t} \log p(\boldy \mid \boldx_t)\\
%	& = \mathbb{E}\left[ \boldx_{0} | \boldx_t\right] + \sigma_{t}^2 \nabla_{\boldx_t} \log p(\boldy \mid \boldx_t)
%\end{align*}


%And. DDS \cite{chung2024decomposed} makes the assumption that the tangent space at the denoised sample forms a Krylov subspace, allowing efficient data consistency updates via conjugate gradient steps \cite{chung2024decomposed}.
%In a more general way, \cite{zhu_denoising_2023} propose to approximate with 
%\begin{equation}\label{eq:bayes2}
%	\nabla_{\boldz_t} \log p(\boldy \mid \boldz_t) = \frac{1}{\sigma_{t}}(\mathbb{E}\left[ \boldx_{0} | \boldx_t, \boldy\right] - \mathbb{E}\left[ \boldx_{0} | \boldx_t\right])
%\end{equation}
%Inspired by previous works \cite{zhu_denoising_2023,chung2024decomposed}, we use the proximal update to approximate the conditional posterior mean
